Efficient Transformer Knowledge Distillation: A Performance Review

As pretrained transformer language models continue to achieve state-of-the-art performance, the Natural Language Processing community has pushed for advances in model compression and efficient attention mechanisms to address high computational requirements and limited input sequence length. Despite these separate efforts, no investigation has been done into the intersection of these two fields. In this work, we provide an evaluation of model compression via knowledge distillation on efficient attention transformers. We provide cost-performance trade-offs for the compression of state-of-the-art efficient attention architectures and the gains made in performance in comparison to their full attention counterparts. Furthermore, we introduce a new long-context Named Entity Recognition dataset, GONERD, to train and test the performance of NER models on long sequences. We find that distilled efficient attention transformers can preserve a significant amount of original model performance, preserving up to 98.6% across short-context tasks (GLUE, SQUAD, CoNLL-2003), up to 94.6% across long-context Question-and-Answering tasks (HotpotQA, TriviaQA), and up to 98.8% on long-context Named Entity Recognition (GONERD), while decreasing inference times by up to 57.8%. We find that, for most models on most tasks, performing knowledge distillation is an effective method to yield high-performing efficient attention models with low costs.

==> tables/ablation_compression_methods.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{c}{\textbf{Distillation}} & \multicolumn{2}{c}{\textbf{Pruning}} & \multicolumn{2}{c}{\textbf{Quantization}} & \multirow{2}{*}{\textbf{GLUE}} & \multirow{2}{*}{\textbf{GONER}} \\
\todo{M1} & \todo{M2} & \todo{M1} & \todo{M2} & \todo{M1} & \todo{M2} & \\ 
\hline
\cmark & & \cmark & & & & \todo{*} & \todo{*} \\
& \cmark & \cmark & & & \cmark & \todo{*} & \todo{*} \\
\cmark & & & & & \cmark & \todo{*} & \todo{*} \\
& \cmark & & \cmark & & \cmark & \todo{*} & \todo{*} \\
& \cmark & & \cmark & & \cmark & \todo{*} & \todo{*} \\
& \cmark & & \cmark & \cmark & & \todo{*} & \todo{*} \\
\hline
\end{tabular}
\caption{Ablation on different compression methods used}
\label{table:ablation_methods}
\end{center}
\end{table*}

==> tables/gonerd_sentiment.tex <==
\begin{figure}[h!]
    \begin{minipage}{0.2\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}ccc@{}}
        \hline
        Sentiment & \# & $p$ \Tstrut\Bstrut\\
        \hline
        Positive & * & *\Tstrut\\
        Neutral & * & * \\
        Negative & * & * \Bstrut\\
        \hline
        \textbf{Total} & * & 1 \Tstrut\Bstrut\\
        \hline
        \\
        \hline
        Domains & \# & $p$ \Tstrut\Bstrut\\
        \hline
        justice.gov & * & *\Tstrut\\
        justice.gov & * & * \\
        justice.gov & * & * \\
        justice.gov & * & * \\
        justice.gov & * & * \Bstrut\\
        \hline
        \textbf{Total} & * & 1 \Tstrut\Bstrut\\
        \hline
    \end{tabular}
    }
    \end{minipage}
    \begin{minipage}{0.8\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/gonerd_transfer/sentiment_distribution.png}
    \end{minipage}%
\caption{sentiment distribution, sentiment counts, stop words}
\label{fig:test}
\end{figure}

==> tables/gonerd_stopwords.tex <==
\begin{table}[h!]
\setlength{\belowcaptionskip}{-15pt}
\setlength{\tabcolsep}{1pt}
\begin{center}
{\scriptsize
\begin{tabular}{lccccccccccc}
\hline 
 \\[-.2cm]
\raisebox{.4cm}{p} & \rotatebox{68}{\textbf{word 1}} & \rotatebox{68}{\textbf{word 2}} & \rotatebox{68}{\textbf{word 3}} & \rotatebox{68}{\textbf{word 4}} & \rotatebox{68}{\textbf{word 5}} & \rotatebox{68}{\textbf{word 6}} & \rotatebox{68}{\textbf{word 7}} & \rotatebox{68}{\textbf{word 8}} & \rotatebox{68}{\textbf{word 9}} & \rotatebox{68}{\textbf{word 10}} \Tstrut\Bstrut\\
\hline \Tstrut
pdf & * & * & * & * & * & * & * & * & * & * \\ \Bstrut
cdf & * & * & * & * & * & * & * & * & * & * \\
\hline
\end{tabular}
\vspace{.3cm}
\caption{\todo{*}}
\label{table:gonerd_stopwords}
}
\end{center}
\end{table}

==> tables/gonerd_summary.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.37\linewidth}
    \centering       
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c@{\hskip .5cm}c@{\hskip .7cm}c@{\hskip .7cm}c@{\hskip 1cm}c@{\hskip .7cm}c@{\hskip .7cm}c@{\hskip .5cm}}
    \hline
    \multirow{2}{*}{Type} & \multicolumn{3}{c}{\hspace{-1.1cm}\textbf{GONERD} (4096)} & \multicolumn{3}{c}{\hspace{-.7cm}\textbf{CoNLL-2003} (512)} \Tstrut\\
     & \# & $p$ & $p^1$ & \# & $p$ & $p^1$ \Bstrut\\
    \hline
    O & * & * & - & * & * & - \Tstrut\\
    B-PER & * & * & * & * & * & * \\
    I-PER & * & * & * & * & * & * \\
    B-ORG & * & * & * & * & * & * \\
    I-ORG & * & * & * & * & * & * \\
    B-LOC & * & * & * & * & * & * \\
    I-LOC & * & * & * & * & * & * \\
    B-MISC & * & * & * & * & * & * \\
    I-MISC & * & * & * & * & * & * \Bstrut\\
    \hline
    \textbf{Total} & * & 1 & 1 & * & 1 & 1 \Tstrut\Bstrut\\
    \hline
    \end{tabular}
    }
    \label{table:asdf}
    \end{minipage}
    \quad
    \begin{minipage}{0.63\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholders/length_compare.PNG}
    \end{minipage}%
    \caption{token type counts and sample length distribution comparisons, $p^1$ indicates probability with removal of "O" token}
\end{figure*}

==> tables/summary_distill_convert.tex <==
\begin{table}[H]
\setlength{\belowcaptionskip}{-15pt}
\setlength{\tabcolsep}{3pt}
\begin{center}
{\footnotesize
\begin{tabular}{l@{\hskip .13cm}ccccc}
\cline{2-6} \\[-.2cm]
& \raisebox{.5cm}{Dataset} & \rotatebox{65}{\textbf{RoBERTA}} & \rotatebox{65}{\textbf{$\Delta$ KD}} & \rotatebox{65}{\textbf{$\Delta$ \textit{Convert}}} & \rotatebox{65}{\textbf{$\Delta$ \textit{Convert}+KD}} \Tstrut\Bstrut\\
\cline{2-6} \Tstrut
\multirow{5}{*}[-0.4ex]{\rotatebox{90}{\textbf{512}}} & Inf. Time (sec.) & .148 & -39.9\% & +0.7\% & \textbf{-49.3\%} \\
& GPU Mem. & 4843 & -3.7\% & -15.8\% & \textbf{-20.4\%} \\[.1cm]
& GLUE & 83.17 & -7.3\% & +0.7\% & \textbf{-7.8\%} \\
& SQuAD1.1 & 92.47 & -5.0\% & -2.5\% & \textbf{-7.0\%} \\ \Bstrut
& CoNLL-2003 & 93.43 & +0.5\% & +0.3\% & \textbf{+0.2\%} \\
\cline{2-6} \Tstrut
\multirow{5}{*}[-0.3ex]{\rotatebox{90}{\textbf{4096}}} & Inf. Time (sec.) & 1.886 & 0.798 & 1.110 & \textbf{0.588} \\
& GPU Mem. & 42506 & 42326 & 11881 & \textbf{11661} \\[.1cm]
& HotpotQA & - & - & 73.48 & \textbf{-11.6\%} \\
& TriviaQA & - & - & 60.52 & \textbf{-15.0\%} \\ \Bstrut
& GONERD & - & - & 70.6 & \textbf{-4.1\%} \\
\cline{2-6}
\end{tabular}
\vspace{.3cm}
\caption{Effects of introducing Knowledge Distillation and Longformer attention into RoBERTa on various tasks. We report average score for GLUE and overall F1 for QA and NER. "$\Delta$" indicates a change from the base model. Results are compared against RoBERTa on short-context tasks and against Longformer ($\Delta$ \textit{Convert}) on long-context tasks. Sequence lengths of 512 are used for inference time and memory usage.}
\label{table:summary_convert_distill}
}
\end{center}
\end{table}
